On False Data Injection Attack against Building Automation Systems

KNX is one popular communication protocol for a building automation system (BAS). However, its lack of security makes it subject to a variety of attacks. We are the first to study the false data injection attack against a KNX based BAS. We design a man-in-the-middle (MITM) attack to change the data from a temperature sensor and inject false data into the BAS. We model a BAS and analyze the impact of the false data injection attack on the system in terms of energy cost. Since the MITM attack may disturb the KNX traffic, we design a machine learning (ML) based detection strategy to detect the false data injection attack using a novel feature based on the Jensen Shannon Divergence (JSD), which measures the similarity of KNX telegram inter-arrival time distributions with attack and with no attack. We perform real-world experiments and validate the presented false data injection attack and the ML based detection strategy. We also simulate a BAS, and show that the false data injection attack has a huge impact on the BAS in terms of power consumption.

==> sections/Discussion.tex <==
% Section
\section{Discussion}
\label{Discussion}


In our attack, the DXR2 does not seem to perform any authentication to a device writing to the logical tag. Possible defense measures could include an authentication check before the data from the Telegram is converted to a BACnet property value.


==> sections/Telegram.tex <==
% Section
\vspace{-2mm}
\subsection{Crafting a KNX Telegram}
\label{Telegram}
\vspace{-2mm}

\Shan{It's better to move this section after Eavesdropping Attack, so as to introduce the attack workflow step by step.}

To perform replay and impersonation attacks, we need to craft KNX telegrams. Figure \ref{fig:LTEvsStd} illustrates the structures of the standard and extended KNX TP1 frames. 
%This section introduces and compares the two types of frames.
% \Michael{Previous sections introduced concepts of attack. I think our explanation of our attack should be in its own section before evaluation}
% \Fu{This part may be moved to the subsection of Setup of Section Evaluation.}
% \Michael{Moved to subsection of setup of Section Evaluation}
%Once the structure of a frame is obtained, desired standard or extended telegrams can be crafted.
%Here, we explain each field in a KNX TP1 frame for both standard and extended frames.
We now introduce a few fields critical to our physical-cyber attacks.


% % \subsection{Crafting a Telegram}
% \subsubsection{Control Field}
% For the control field, there are 8 bits, we denote as D7-D0 from left to right. Starting with the control field, the first bit D7 details the telegram type. Standard KNX frames set this bit to 1 while an extended KNX frame sets this bit to 0. This is one of the significant differences between the two types of frames, as setting the telegram type bit to 0 signifies that the next field following the control field should be the extended control field and the max length of the frame can be longer than the standard's max of 22 octets. If the telegram type bit is set to 1 for standard frames, the source address is instead the next field to follow. Bit D5 is the telegram repetition status. A value of 0 signifies that the telegram being built is a repetition of a previous telegram, where a value of 1 signifies an original telegram. Finally, bits D3 and D2 are coupled together to represent the telegram priority. There are four priority levels: system (00), urgent (10), normal (01), and low (00). Bits D6, D4, D1, D0 are fixed to 0, 1, 0, 0, respectively. These values are always set for these bits in every KNX frame, no matter if they are standard or extended. 

%\vspace{-2mm}
%\subsubsection{Extended Control Field}
{\bf Extended Control Field}:
The extended control field is the second octet in a KNX LTE frame. It can be divided in three parts: the address type, hop count, and Extended Frame Format (EFF). The address type is 1 bit in length and describes whether the destination is either a group or individual address. The hop count, which is 3 bits and follows the address type, limits the distance the telegram can travel to ensure it does not endlessly traverse the KNX network. By default, this value is set to 6 for multicast telegrams. This value is decremented as it traverses the network. Unicast and broadcast telegrams are sent with a hop count value of 7 and are never decremented during transmission. Finally, the EFF are the last 4 bits of the octet. The EFF describes what type of format that should be used for the destination address. It can be a standard frame format for a standard group/individual address, an extended frame format for a standard group/individual address, or an LTE extended address type. For an LTE extended address type, the first two bits indicate that it is of this type and the last two bits describe what type of LTE extension the destination address should be interpreted as. This can be either a geographical tag for lower level apartment/floors (EFF of 0100), geographical tags for upper level apartment/floors (EFF of 0101), application specific tags (EFF of 0110), or unassigned/broadcast tags (EFF of 0111). Depending on this extension, the bit interpretation of the destination address differs to represent the logical tag address.

%\vspace{-2mm}
%\subsubsection{Source Address}
{\bf Source Address}:
The source address follows the control field in a standard KNX frame, and follows the extended control field in an extended KNX frame. With a size of 2 octets, this is the individual address of the device that is sending the telegram.

%\vspace{-2mm}
%\subsubsection{Destination Address}
{\bf Destination Address}:
A destination address of 2 octets follows the source address. Based on the address type bit, the destination can be either an individual address or a group address. When the address bit is 0, the destination is an individual address and the telegram will then be a unicast message. An address bit of 1 declares the destination as a group address for multicast or broadcast communication. For standard telegram frames, bit representation of the group address follows that from section \ref{Background}. KNX extended telegrams used the bit representation selected from the EFF field in the extended control field.

% \subsubsection{Address Type, Hop Count, and Length}
% The next octet differs for standard and extended frames. For standard frames, the first 4 bits are the address type (1 bit) and hop count (3 bits), respectively. The last 4 bits are used to declare how long the payload will be for the telegram. Recall that the address type and hop count for extended frames are in the extended control field instead of in this octet. This is because for extended frames, the whole octet is used for the length of the data since extended frames are longer than standard frames. So, using all 8 bits of the octet is required to describe how long the telegram's payload is for the extended frame. \looseness=-1

% \subsubsection{Transport Protocol Data Unit (TPDU)}
% Octet 6 for standard frames and octet 7 for extended frames are the start of the the Transport Protocol Data Unit (TPDU). The Transport Protocol Control Information (TPCI) is the first 6 bits of the TPDU. The first two bits of the TPCI indicate the type of communication in the transport layer. This can be either a Unnumbered Data Packet (UDP with coding 00), a Numbered Data Packet (NDP with code 01), Unnumbered Control Data (UCD with code 10), or a Numbered Control Data (NCD with code 11). The last 4 bits specify the sequence number, but only if the communication is one of the numbered types. For unnumbered communication, these 4 bits are all set to 0. \looseness=-1

% The last two bits in this octet have different significance for an UCD, NCD, or unnumbered communication. When an UCD is signified, the last 2 bits are either for when a point-to-point connection is opened (00) or when the point-to-point connection is terminated (01). The NCD's last two bits of this octet positively confirm (10) or negatively confirm (11) the reception of a previously transmitted telegram. For unnumbered UDP or NDP, the two bits are the start of the Application Protocol Control Information (APCI). The APCI code uses the last 2 bits in this octet and the next 2 bits of the following (octet 7 for standard and 8 for extended). This code distinguishes the application service for the telegram, such as a \texttt{GroupValueRead}, \texttt{GroupValueWrite}, or \texttt{Restart} service. For extended LTE, their APCI are 10 bits to distinguish their application service, such as for \texttt{GroupPropertyValueInfoReport} (1111101011). If the length of the payload is 6 bits or shorter, it is encoded in the remainder of this octet. When the payload is larger than 6 bits, these bits are all set to 0 and the payload begins in a new octet after. 

% For LTE devices, following the APCI are the OT (2 octets), the OI (1 octet), and the PID (1 Octet). The data for the payload would instead trail after the PID, starting in a new octet.

% \subsubsection{Checksum}
% Standard lengths range from 9 octets to a maximum of 22 octets. Extended frames can reach a maximum of 254 octets. The end of each telegram includes the checksum octet. This checksum is based on the NOT XOR logical function used over the previous octets in the telegram.



% \Fu{Are any of the following items not presented yet? Please provide details. You guys spent so much time on it. For example, how did you craft the correct LTE telegram?}

% \begin{itemize}
%   \item Describe Replay attack
%   \begin{itemize}
%       \item how the the program performs the bus monitoring
%       \item what it data is pulled from the KNX bus (Telegrams)
%       \item what type of information is taken from telegram
%       \item how the new Telegram is built with the capture information
%       \item how it sends the telegram with the same details onto the bus
%   \end{itemize}
%   \item Replay attack for standard KNX devices and controllers
%   \item Adjustments for replay attack on KNX-LTE devices and controllers
%   \item What is Siemen's KNX Peripherial Link (PL-Link) protocol
%   \item How does KNX PL-Link change replay attack approach
%   \item Possibly include algorithm
% \end{itemize}

==> sections/sec7_RelatedWork.tex <==
% Section
\section{Related Work}
\label{relatedwork}

% \begin{itemize}
%   \item papers to cover:
% \end{itemize}

% In this section, we introduce related work on attacks on KNX.

Lopez-Aguilar et. al \cite{Aguilar_2019} designed an emulation for KNX telegrams using MATLAB/Simulink, where their program correctly emulated KNXnet/IP protocol communication and was able to create a communication between the the MATLAB/Simulink and a KNX control board. The MATLAB/Simulink program was able to send and receive KNXnet/IP telegrams and validated their work by monitoring data packets traffic using Wireshark. Using Wireshark, they captured connection requests and responses sent to and from the MATLAB/Simulink program and KNX device.

Antonini et. al \cite{Antonini2015A_Practical} analyzed possible attack scenarios on building automation systems. Using KNXnet/IP, they demonstrate feasible attacks on a full-fledged KNX testbed. By sniffing the traffic messages for programming an actuator in their testbed, they were able to manually identify the hex codes that are used for reprogramming and executing commands for the actuator. These can be replayed back to the actuator. If the system is protected by a password, an attacker can simulate a malfunction, such as constantly changing actuator positions. This type of command is not authenticated, so system administrators would reprogram the device by sending the password used to protect the system. This password is sent in plaintext, so sniffing the traffic will reveal the password to the attack. This allows for the reprogramming and well as changing of the password.

In \cite{wyss_sholander_darby_phelan_2007}, Wyss et. al define the combination of physical attacks and cyber attacks, which they call blended cyber-physical attacks. A cyber-enabled physical attack uses a cyber attack as a pathway for enabling a follow-up physical attack in order to manipulate or disrupt a physical component. On the contrary, a physical-enabled cyber attack use a physical attack to gain access to a cyber control point in order to conduct the following cyber attack. Ways to minimize the potential of a blended attack were to implement the best practices for both physical and cyber attacks as well as to understand the interactions between the physical and cyber components of a system in order to identify potential vulnerabilities.

A survey on the security of Cyber-Physical Systems was conducted by Humayed et. al in \cite{HLLL:CPSSecurity:Survey}. 

A python library called Boiboite Open Framework (BOF) was created by Vacherot \cite{vacherot:hal-03022310} that supports creation, parsing, and manipulation of frames in the KNXnet/IP protocol. The intention was to create a library that does not require the end user to have extensive knowledge in the KNX protocol in order to use it. They test BOF on two threats that target Building Management Systems (BMS): (1) degrading a BMS through the use of normal KNX features and (2) discovering vulnerabilities using malicious frames. Using fuzzing techniques, they generate test frames with mutated inputs in order to observe the behavior. Out of approximately 1.2 million test frames sent in one hour to a testing device, they were able to trigger 20 unexpected behaviors from the device. They approach only observes what is seen client-side. Monitoring target-side as well is mentioned in improving the interpretation of the results.

A novel approach to specification-based intrusion detection system (IDS) for network controlled systems is presented in \cite{197145}. Specifically, they introduce an IDS that automates the creation of specification rules using the same documentation that administrators use to maintain the system. They design this approach for a BACnet building automation system and test it on two real-world environments. Their results showed that this specification-based IDS was effective in identifying intrusions, such as dangerous misconfigurations. It also improves on the time to develop and deploy the IDS.

In \cite{8718149}, a risk analysis is conducted for different segments of a field bus, using KNX as a example field bus. They calculate the risk of a segment using a vector which contains static and dynamic data. Some static values include: (1) the class of affiliated devices physical access of attached devices, (2) physical access of used wires, (3) reachability of other clients, (4) type of telegrams and (5) reachability to other clients. While some dynamic values of the vector are: (1) the type of telegrams and (2) the number of telegrams per time slot. Classification is done for the static data used for the static risk analysis. Using this classification, they can calculate a risk percentage for further evaluation of the field bus segment. They mention possible strategies for defense which include using an intrusion detection system, static risk minimization for systems not yet deployed, and KNX-Secure.

% Glanzer et. al

Molina \cite{molina2014} used his hotel room's ipad, which uses a preloaded application for controlling the KNX room devices, to access his room's KNX network. By reverse engineering the KNXnet/IP protocol and monitoring the KNX traffic using Wireshark, he identified the addresses of the devices in the hotel room. Using this information, Molina manipulated each KNX device remotely without the need of the hotel ipad. Not only did he find his room devices's addresses to communicate to, he was also able to communicate with devices in other hotel rooms.

Rios demos in \cite{Rio::FacilityManagementSystems::2014} several attacks to exploit and gain access to facility management systems. In the Niagara Framework, Rios shows that it is vulnerable to password retrieval attacks by unauthenticated users. A routine was written to decode the encoded password, where the now plaintext password can be used to gain administrative acess to the device. The Metasys building automation system is also shown to be susceptible to device password retrievals by unauthenticated users, as well as reset the password for any user, providing a bypass for the authentication process, which will compromise the system.

Previous study of communicating between the KNX and BACnet communication protocols includes Kastner and Szucsich \cite{kastner2011}, where they designed a data model that maps KNX into BACnet Web Services (BACnet/WS). BACnet/WS is a web service based standard that facilitates integration for building automation systems and IT networks. Their model maps the datapoint types, like binary inputs for switches, and communication services, such as request-based and spontaneous transmissions. In the request-based transmission, group objects are essentially states, where the BACnet/WS server has the ability to obtain the current readings for those group objects. Spontaneous transmission are event-driven, where incoming events causes an update in the server. To implement access to the KNX network, they use the Calimero java library for KNX applications \cite{calimero_project}. Overall, their model demonstrates the ability to transmit KNX data and commands across building automation protocols.

Granzer et. al \cite{Grazner_2008} present an approach to integrate KNX and BACnet field networks together through the use of multi-protocol devices, named a BACknx device. These devices implement the protocol stacks of both BACnet and KNX and uses KNX as the transport medium for both. Four distinct tables are created for mapping object ID, property ID, the object type, and the property type. BACnet objects are mapped to KNX equivalents. Their proof-of-concept demonstrated this BACknx device using a prototype BACnet inter-network with a BACnet/Ethernet backbone and KNX TP1 medium. These two protocols are then connected through a BACnet/Ethernet-to-BACnet/KNX router, which takes either a BACnet/KNX or BACnet/Ethernet message and converts it to the second protocol prior to transmitting it to its correct destination.

% monitors captured KNX traffic from a hotel iPad to KNX devices in the room to discover the room's KNX devices and their associated addresses by reverse engineering the KNX/IP protocol.
% The hotel iPad contains a pre-loaded application designed to control the room devices, such as lights, blinds, and TV. Monitoring the traffic generated by the application also allowed him to learn commands used to control each KNX device. With knowledge of the address for each KNX device in the hotel room and the commands used to control them, Molina was able to manipulate every KNX device remotely, without the use of the hotel iPad. 

% \subsection{}

